On the Role of Diversity in Sparsity Estimation

A major challenge in sparsity pattern estimation is that small modes are difficult to detect in the presence of noise. This problem is alleviated if one can observe samples from multiple realizations of the nonzero values for the same sparsity pattern. We will refer to this as "diversity". Diversity comes at a price, however, since each new realization adds new unknown nonzero values, thus increasing uncertainty. In this paper, upper and lower bounds on joint sparsity pattern estimation are derived. These bounds, which improve upon existing results even in the absence of diversity, illustrate key tradeoffs between the number of measurements, the accuracy of estimation, and the diversity. It is shown, for instance, that diversity introduces a tradeoff between the uncertainty in the noise and the uncertainty in the nonzero values. Moreover, it is shown that the optimal amount of diversity significantly improves the behavior of the estimation problem for both optimal and computationally efficient estimators.

==> inkscape-figs/figures.tex <==
%LaTeX with PSTricks extensions
%%Creator: inkscape 0.48.0
%%Please note this file requires PSTricks extensions
\psset{xunit=.5pt,yunit=.5pt,runit=.5pt}
\begin{pspicture}(360,180)
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=1.65434039,linecolor=curcolor]
{
\newpath
\moveto(35,25)
\lineto(35,25)
\lineto(35,155)
\lineto(50,155)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=2,linecolor=curcolor]
{
\newpath
\moveto(35.417912,155)
\lineto(70,155)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(74.616,155)
\lineto(67.696,151)
\lineto(67.696,159)
\lineto(74.616,155)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=1,linecolor=curcolor]
{
\newpath
\moveto(74.616,155)
\lineto(67.696,151)
\lineto(67.696,159)
\lineto(74.616,155)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=2,linecolor=curcolor]
{
\newpath
\moveto(20,85)
\lineto(35,85)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(9.89592614,93.45468184)
\lineto(9.89592614,90.93697131)
\curveto(9.20368367,91.40556431)(8.55057727,91.75489097)(7.936605,91.98495234)
\curveto(7.32261686,92.21497974)(6.72970461,92.33000194)(6.15786646,92.33001927)
\curveto(5.16465703,92.33000194)(4.39718177,92.05735674)(3.85543839,91.51208285)
\curveto(3.31970671,90.96677594)(3.0518428,90.19144115)(3.05184585,89.18607616)
\curveto(3.0518428,88.34256588)(3.2294155,87.7035537)(3.5845645,87.26903768)
\curveto(3.94572574,86.84301728)(4.6259195,86.4979507)(5.62514781,86.2338369)
\lineto(6.72670163,85.91433048)
\curveto(8.08708241,85.54795258)(9.0893148,84.90042023)(9.73340181,83.97173149)
\curveto(10.38348876,83.05154497)(10.70853711,81.8161214)(10.70854782,80.26545709)
\curveto(10.70853711,78.41657656)(10.2691199,77.01500983)(9.39029488,76.06075269)
\curveto(8.5174705,75.10649343)(7.23533536,74.62936433)(5.54388564,74.62936396)
\curveto(4.90582224,74.62936433)(4.22562848,74.73160628)(3.50330233,74.93609011)
\curveto(2.78698859,75.14057408)(2.04359099,75.44303985)(1.2731073,75.84348833)
\lineto(1.2731073,78.50178169)
\curveto(2.01349392,77.91388697)(2.73883328,77.47083852)(3.44912755,77.17263501)
\curveto(4.15941493,76.87442715)(4.85766693,76.7253243)(5.54388564,76.72532603)
\curveto(6.58523868,76.7253243)(7.38883041,77.01500983)(7.95466326,77.59438347)
\curveto(8.5204802,78.17375193)(8.80339265,79.00020769)(8.80340145,80.07375324)
\curveto(8.80339265,81.01096605)(8.59873258,81.74370002)(8.18942064,82.27195737)
\curveto(7.78611172,82.80020017)(7.1209665,83.19638773)(6.19398298,83.46052123)
\lineto(5.08340003,83.76724738)
\curveto(3.72300743,84.15064593)(2.73883328,84.75131739)(2.13087462,85.56926356)
\curveto(1.5229117,86.38718859)(1.2189313,87.52463028)(1.21893252,88.98159205)
\curveto(1.2189313,90.66857025)(1.63728056,91.9977156)(2.47398155,92.9690321)
\curveto(3.316697,93.94031265)(4.47543415,94.42596192)(5.95019647,94.42598134)
\curveto(6.58222897,94.42596192)(7.22630624,94.34502037)(7.88243023,94.18315647)
\curveto(8.53853844,94.0212542)(9.20970308,93.77842956)(9.89592614,93.45468184)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=2,linecolor=curcolor]
{
\newpath
\moveto(35.417912,105)
\lineto(70,105)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(74.616,105)
\lineto(67.696,101)
\lineto(67.696,109)
\lineto(74.616,105)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=1,linecolor=curcolor]
{
\newpath
\moveto(74.616,105)
\lineto(67.696,101)
\lineto(67.696,109)
\lineto(74.616,105)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=2,linecolor=curcolor]
{
\newpath
\moveto(35.417912,25)
\lineto(70,25)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(74.616,25)
\lineto(67.696,21)
\lineto(67.696,29)
\lineto(74.616,25)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=1,linecolor=curcolor]
{
\newpath
\moveto(74.616,25)
\lineto(67.696,21)
\lineto(67.696,29)
\lineto(74.616,25)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(90.14873771,164.31387025)
\lineto(86.49194019,157.34863043)
\lineto(90.33834943,149.99998292)
\lineto(88.37902829,149.99998292)
\lineto(85.43553201,155.6232958)
\lineto(82.49203574,149.99998292)
\lineto(80.5327146,149.99998292)
\lineto(84.46038601,157.48921326)
\lineto(80.8667924,164.31387025)
\lineto(82.82611354,164.31387025)
\lineto(85.50776505,159.21454789)
\lineto(88.18941657,164.31387025)
\lineto(90.14873771,164.31387025)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(93.23670006,152.17262653)
\lineto(96.21631285,152.17262653)
\lineto(96.21631285,166.72933874)
\lineto(92.9748553,165.80916027)
\lineto(92.9748553,168.16072747)
\lineto(96.19825459,169.08090594)
\lineto(98.02213879,169.08090594)
\lineto(98.02213879,152.17262653)
\lineto(101.00175158,152.17262653)
\lineto(101.00175158,149.99998292)
\lineto(93.23670006,149.99998292)
\lineto(93.23670006,152.17262653)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(90.14873771,114.3138759)
\lineto(86.49194019,107.34863608)
\lineto(90.33834943,99.99998857)
\lineto(88.37902829,99.99998857)
\lineto(85.43553201,105.62330145)
\lineto(82.49203574,99.99998857)
\lineto(80.5327146,99.99998857)
\lineto(84.46038601,107.48921891)
\lineto(80.8667924,114.3138759)
\lineto(82.82611354,114.3138759)
\lineto(85.50776505,109.21455354)
\lineto(88.18941657,114.3138759)
\lineto(90.14873771,114.3138759)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(94.49174908,102.17263218)
\lineto(100.8572855,102.17263218)
\lineto(100.8572855,99.99998857)
\lineto(92.29767057,99.99998857)
\lineto(92.29767057,102.17263218)
\curveto(92.9899018,103.18652935)(93.93194005,104.54549527)(95.12378816,106.24953402)
\curveto(96.32164732,107.96208044)(97.07407404,109.06544148)(97.38107058,109.55962047)
\curveto(97.96494728,110.48830862)(98.37125771,111.27216357)(98.60000308,111.91118767)
\curveto(98.83475257,112.55870811)(98.95213113,113.19346022)(98.95213914,113.81544589)
\curveto(98.95213113,114.82933142)(98.69931576,115.65578718)(98.19369225,116.29481566)
\curveto(97.69407366,116.93381156)(97.04096726,117.25331765)(96.23437111,117.2533349)
\curveto(95.66252151,117.25331765)(95.05757043,117.11273497)(94.41951604,116.83158644)
\curveto(93.78747412,116.55040424)(93.11029007,116.12439612)(92.38796187,115.55356078)
\lineto(92.38796187,118.16073312)
\curveto(93.1223289,118.57820292)(93.80854207,118.89344893)(94.44660343,119.1064721)
\curveto(95.08465779,119.31945706)(95.66854092,119.42595909)(96.19825459,119.42597852)
\curveto(97.59475333,119.42595909)(98.70834488,118.93178967)(99.53903257,117.94346876)
\curveto(100.36970308,116.95511196)(100.78504263,115.63448677)(100.78505247,113.98158923)
\curveto(100.78504263,113.1977203)(100.67970288,112.45220608)(100.46903293,111.74504433)
\curveto(100.26436333,111.04637926)(99.88814997,110.2199235)(99.34039172,109.26567457)
\curveto(99.18989798,109.01858059)(98.71135458,108.30288694)(97.9047601,107.11859147)
\curveto(97.09815169,105.94280192)(95.96048249,104.29415048)(94.49174908,102.17263218)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(90.14873771,34.31386315)
\lineto(86.49194019,27.34862334)
\lineto(90.33834943,19.99997583)
\lineto(88.37902829,19.99997583)
\lineto(85.43553201,25.6232887)
\lineto(82.49203574,19.99997583)
\lineto(80.5327146,19.99997583)
\lineto(84.46038601,27.48920616)
\lineto(80.8667924,34.31386315)
\lineto(82.82611354,34.31386315)
\lineto(85.50776505,29.21454079)
\lineto(88.18941657,34.31386315)
\lineto(90.14873771,34.31386315)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(92.75815618,39.08089884)
\lineto(94.58204038,39.08089884)
\lineto(94.58204038,21.32912251)
\curveto(94.58203674,19.0286773)(94.27203693,17.35872545)(93.65204002,16.31926194)
\curveto(93.03805711,15.2798058)(92.04786354,14.76007588)(90.68145636,14.76007064)
\lineto(89.98621337,14.76007064)
\lineto(89.98621337,16.93271426)
\lineto(90.55504854,16.93271426)
\curveto(91.36165037,16.93271732)(91.93048498,17.25222342)(92.26155405,17.8912335)
\curveto(92.59262049,18.53024779)(92.75815437,19.67620965)(92.75815618,21.32912251)
\lineto(92.75815618,39.08089884)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=2,linecolor=curcolor]
{
\newpath
\moveto(105.417912,155)
\lineto(139.999997,155)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(144.615997,155)
\lineto(137.695997,151)
\lineto(137.695997,159)
\lineto(144.615997,155)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=1,linecolor=curcolor]
{
\newpath
\moveto(144.615997,155)
\lineto(137.695997,151)
\lineto(137.695997,159)
\lineto(144.615997,155)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=2,linecolor=curcolor]
{
\newpath
\moveto(105.417915,105)
\lineto(139.999997,105)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(144.615997,105)
\lineto(137.695997,101)
\lineto(137.695997,109)
\lineto(144.615997,105)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=1,linecolor=curcolor]
{
\newpath
\moveto(144.615997,105)
\lineto(137.695997,101)
\lineto(137.695997,109)
\lineto(144.615997,105)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=2,linecolor=curcolor]
{
\newpath
\moveto(105.417923,25)
\lineto(139.999997,25)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(144.615997,25)
\lineto(137.695997,21)
\lineto(137.695997,29)
\lineto(144.615997,25)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=1,linecolor=curcolor]
{
\newpath
\moveto(144.615997,25)
\lineto(137.695997,21)
\lineto(137.695997,29)
\lineto(144.615997,25)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(149.96388739,169.08090594)
\lineto(151.92320853,169.08090594)
\lineto(155.66126822,161.23382842)
\lineto(159.37224052,169.08090594)
\lineto(161.33156166,169.08090594)
\lineto(156.56418119,159.08674532)
\lineto(156.56418119,149.99998292)
\lineto(154.73126786,149.99998292)
\lineto(154.73126786,159.08674532)
\lineto(149.96388739,169.08090594)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(163.59787321,152.17262653)
\lineto(166.577486,152.17262653)
\lineto(166.577486,166.72933874)
\lineto(163.33602845,165.80916027)
\lineto(163.33602845,168.16072747)
\lineto(166.55942774,169.08090594)
\lineto(168.38331194,169.08090594)
\lineto(168.38331194,152.17262653)
\lineto(171.36292473,152.17262653)
\lineto(171.36292473,149.99998292)
\lineto(163.59787321,149.99998292)
\lineto(163.59787321,152.17262653)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(175.24545049,153.24616808)
\lineto(177.15059685,153.24616808)
\lineto(177.15059685,151.04796396)
\lineto(175.66981959,146.95828186)
\lineto(174.50506186,146.95828186)
\lineto(175.24545049,151.04796396)
\lineto(175.24545049,153.24616808)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(185.28584269,166.53763489)
\lineto(182.81186116,157.04190428)
\lineto(187.76885335,157.04190428)
\lineto(185.28584269,166.53763489)
\moveto(184.25652191,169.08090594)
\lineto(186.32419261,169.08090594)
\lineto(191.46176739,149.99998292)
\lineto(189.56565016,149.99998292)
\lineto(188.33768852,154.89482118)
\lineto(182.26108425,154.89482118)
\lineto(181.03312261,149.99998292)
\lineto(179.10991799,149.99998292)
\lineto(184.25652191,169.08090594)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(193.8996324,152.17262653)
\lineto(196.8792452,152.17262653)
\lineto(196.8792452,166.72933874)
\lineto(193.63778764,165.80916027)
\lineto(193.63778764,168.16072747)
\lineto(196.86118694,169.08090594)
\lineto(198.68507113,169.08090594)
\lineto(198.68507113,152.17262653)
\lineto(201.66468393,152.17262653)
\lineto(201.66468393,149.99998292)
\lineto(193.8996324,149.99998292)
\lineto(193.8996324,152.17262653)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(149.96388739,119.08091159)
\lineto(151.92320853,119.08091159)
\lineto(155.66126822,111.23383407)
\lineto(159.37224052,119.08091159)
\lineto(161.33156166,119.08091159)
\lineto(156.56418119,109.08675097)
\lineto(156.56418119,99.99998857)
\lineto(154.73126786,99.99998857)
\lineto(154.73126786,109.08675097)
\lineto(149.96388739,119.08091159)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(163.59787321,102.17263218)
\lineto(166.577486,102.17263218)
\lineto(166.577486,116.72934439)
\lineto(163.33602845,115.80916592)
\lineto(163.33602845,118.16073312)
\lineto(166.55942774,119.08091159)
\lineto(168.38331194,119.08091159)
\lineto(168.38331194,102.17263218)
\lineto(171.36292473,102.17263218)
\lineto(171.36292473,99.99998857)
\lineto(163.59787321,99.99998857)
\lineto(163.59787321,102.17263218)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(175.24545049,103.24617373)
\lineto(177.15059685,103.24617373)
\lineto(177.15059685,101.04796961)
\lineto(175.66981959,96.95828751)
\lineto(174.50506186,96.95828751)
\lineto(175.24545049,101.04796961)
\lineto(175.24545049,103.24617373)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(185.28584269,116.53764054)
\lineto(182.81186116,107.04190993)
\lineto(187.76885335,107.04190993)
\lineto(185.28584269,116.53764054)
\moveto(184.25652191,119.08091159)
\lineto(186.32419261,119.08091159)
\lineto(191.46176739,99.99998857)
\lineto(189.56565016,99.99998857)
\lineto(188.33768852,104.89482683)
\lineto(182.26108425,104.89482683)
\lineto(181.03312261,99.99998857)
\lineto(179.10991799,99.99998857)
\lineto(184.25652191,119.08091159)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(193.8996324,102.17263218)
\lineto(196.8792452,102.17263218)
\lineto(196.8792452,116.72934439)
\lineto(193.63778764,115.80916592)
\lineto(193.63778764,118.16073312)
\lineto(196.86118694,119.08091159)
\lineto(198.68507113,119.08091159)
\lineto(198.68507113,102.17263218)
\lineto(201.66468393,102.17263218)
\lineto(201.66468393,99.99998857)
\lineto(193.8996324,99.99998857)
\lineto(193.8996324,102.17263218)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(149.96388739,119.08091159)
\lineto(151.92320853,119.08091159)
\lineto(155.66126822,111.23383407)
\lineto(159.37224052,119.08091159)
\lineto(161.33156166,119.08091159)
\lineto(156.56418119,109.08675097)
\lineto(156.56418119,99.99998857)
\lineto(154.73126786,99.99998857)
\lineto(154.73126786,109.08675097)
\lineto(149.96388739,119.08091159)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(163.59787321,102.17263218)
\lineto(166.577486,102.17263218)
\lineto(166.577486,116.72934439)
\lineto(163.33602845,115.80916592)
\lineto(163.33602845,118.16073312)
\lineto(166.55942774,119.08091159)
\lineto(168.38331194,119.08091159)
\lineto(168.38331194,102.17263218)
\lineto(171.36292473,102.17263218)
\lineto(171.36292473,99.99998857)
\lineto(163.59787321,99.99998857)
\lineto(163.59787321,102.17263218)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(175.24545049,103.24617373)
\lineto(177.15059685,103.24617373)
\lineto(177.15059685,101.04796961)
\lineto(175.66981959,96.95828751)
\lineto(174.50506186,96.95828751)
\lineto(175.24545049,101.04796961)
\lineto(175.24545049,103.24617373)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(185.28584269,116.53764054)
\lineto(182.81186116,107.04190993)
\lineto(187.76885335,107.04190993)
\lineto(185.28584269,116.53764054)
\moveto(184.25652191,119.08091159)
\lineto(186.32419261,119.08091159)
\lineto(191.46176739,99.99998857)
\lineto(189.56565016,99.99998857)
\lineto(188.33768852,104.89482683)
\lineto(182.26108425,104.89482683)
\lineto(181.03312261,99.99998857)
\lineto(179.10991799,99.99998857)
\lineto(184.25652191,119.08091159)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(193.8996324,102.17263218)
\lineto(196.8792452,102.17263218)
\lineto(196.8792452,116.72934439)
\lineto(193.63778764,115.80916592)
\lineto(193.63778764,118.16073312)
\lineto(196.86118694,119.08091159)
\lineto(198.68507113,119.08091159)
\lineto(198.68507113,102.17263218)
\lineto(201.66468393,102.17263218)
\lineto(201.66468393,99.99998857)
\lineto(193.8996324,99.99998857)
\lineto(193.8996324,102.17263218)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(149.96388739,39.08093515)
\lineto(151.92320853,39.08093515)
\lineto(155.66126822,31.23385763)
\lineto(159.37224052,39.08093515)
\lineto(161.33156166,39.08093515)
\lineto(156.56418119,29.08677454)
\lineto(156.56418119,20.00001213)
\lineto(154.73126786,20.00001213)
\lineto(154.73126786,29.08677454)
\lineto(149.96388739,39.08093515)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(163.59787321,22.17265575)
\lineto(166.577486,22.17265575)
\lineto(166.577486,36.72936795)
\lineto(163.33602845,35.80918948)
\lineto(163.33602845,38.16075668)
\lineto(166.55942774,39.08093515)
\lineto(168.38331194,39.08093515)
\lineto(168.38331194,22.17265575)
\lineto(171.36292473,22.17265575)
\lineto(171.36292473,20.00001213)
\lineto(163.59787321,20.00001213)
\lineto(163.59787321,22.17265575)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(175.24545049,23.2461973)
\lineto(177.15059685,23.2461973)
\lineto(177.15059685,21.04799317)
\lineto(175.66981959,16.95831108)
\lineto(174.50506186,16.95831108)
\lineto(175.24545049,21.04799317)
\lineto(175.24545049,23.2461973)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(185.28584269,36.5376641)
\lineto(182.81186116,27.04193349)
\lineto(187.76885335,27.04193349)
\lineto(185.28584269,36.5376641)
\moveto(184.25652191,39.08093515)
\lineto(186.32419261,39.08093515)
\lineto(191.46176739,20.00001213)
\lineto(189.56565016,20.00001213)
\lineto(188.33768852,24.89485039)
\lineto(182.26108425,24.89485039)
\lineto(181.03312261,20.00001213)
\lineto(179.10991799,20.00001213)
\lineto(184.25652191,39.08093515)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(193.8996324,22.17265575)
\lineto(196.8792452,22.17265575)
\lineto(196.8792452,36.72936795)
\lineto(193.63778764,35.80918948)
\lineto(193.63778764,38.16075668)
\lineto(196.86118694,39.08093515)
\lineto(198.68507113,39.08093515)
\lineto(198.68507113,22.17265575)
\lineto(201.66468393,22.17265575)
\lineto(201.66468393,20.00001213)
\lineto(193.8996324,20.00001213)
\lineto(193.8996324,22.17265575)
}
}
\end{pspicture}

